CU-Net: Real-Time High-Fidelity Color Upsampling for Point Clouds

Point cloud upsampling is essential for high-quality augmented reality, virtual reality, and telepresence applications, due to the capture, processing, and communication limitations of existing technologies. Although geometry upsampling to densify a point cloud's coordinates has been well studied, the upsampling of the color attributes has been largely overlooked. In this paper, we propose CU-Net, the first deep-learning point cloud color upsampling model that enables low latency and high visual fidelity operation. CU-Net achieves linear time and space complexity by leveraging a feature extractor based on sparse convolution and a color prediction module based on neural implicit function. Therefore, CU-Net is theoretically guaranteed to be more efficient than most existing methods with quadratic complexity. Experimental results demonstrate that CU-Net can colorize a photo-realistic point cloud with nearly a million points in real time, while having notably better visual performance than baselines. Besides, CU-Net can adapt to arbitrary upsampling ratios and unseen objects without retraining. Our source code is available at https://github.com/UMass-LIDS/cunet.

==> backup.tex <==


\begin{table*}[ht]
  \caption{Color upsampling results on the FaceScape dataset.}
%   \vspace{-4mm}
  \centering
  \label{tab:face}
  \begin{tabular}{cccccc}
    \toprule
    Ratio & Method  & PSNR (dB) & Model Size (MB) & CPU Latency (ms) & GPU Latency (ms)\\
    \midrule
    2$\times$ & Devox/NN  & 31.23 & - & \textbf{13.87} & \textbf{1.73} \\
     & KNN &  30.62 & - & 224.37 & - \\
     & WAAN \cite{fractionalsr}  & 31.33 & - & 323.40 & - \\
     & \cunet(ours)  & \textbf{32.09} & 0.77 & 360.57 & 13.02 \\
     \midrule 
     5$\times$ & Devox/NN  & 30.42 & - & \textbf{38.14} & \textbf{4.69} \\
     & KNN  & 30.49 & - & 960.52 & - \\
     & WAAN \cite{fractionalsr}  & 30.65 & - & 1388.81 & -\\
     & \cunet(ours)  & \textbf{31.32} & 3.01 & 722.74 & 22.17 \\
     \midrule 
     10$\times$ & Devox/NN  & 30.37 & - & \textbf{60.07} & \textbf{7.39}\\
     & KNN  & 30.52 & - & 1665.31 & - \\
     & WAAN \cite{fractionalsr}  & 30.43 & - & 2383.21 & - \\
     & \cunet(ours)  & \textbf{31.26} & 3.01 & 875.04 & 29.06 \\
  \bottomrule
\end{tabular}
\end{table*}



\begin{table}[ht]
  \caption{Results of 8$\times$ color upsampling on the MPEG 8i dataset, measured in PSNR (dB).}
%   \vspace{-4mm}
  \centering
  \label{tab:mpeg}
  \begin{tabular}{ccccc}
    \toprule
    Model  & Devox & KNN & WAAN & \cunet\\
    & /NN & & \cite{fractionalsr} & (ours) \\
    \midrule
    Boxer & 38.95 & 39.47 & 39.57 & \textbf{41.30} \\
    LongDress & 29.53 & 29.62 & 29.63 & \textbf{31.06} \\
    Loot & 39.04 & 39.69 & 39.79 & \textbf{42.56} \\
    RedBlack & 34.30 & 34.96 & 35.04 & \textbf{35.90} \\
    Soldier & 34.77 & 35.29 & 35.34 & \textbf{37.86} \\
    ThaiDancer & 27.20 & 26.85 & 26.78 & \textbf{27.91} \\
  \bottomrule
\end{tabular}
\end{table}

\begin{table}[ht]
  \caption{Details of tasks on the FaceScape dataset.}
%   \vspace{-4mm}
  \centering
  \label{tab:data}
  \begin{tabular}{ccc}
    \toprule
    Type & Space & \#Points (upsample scale) \\
    \midrule
    Input & $100^3$ & 25K \\
    2$\times$ output & $200^3$ & 97K ($\sim$4$\times$) \\
    5$\times$ output & $500^3$ &  445K ($\sim$18$\times$)\\
    10$\times$ output & $1000^3$ & 782K ($\sim$31$\times$)\\
  \bottomrule
\end{tabular}
\end{table}


\begin{figure*}[ht]
  \centering
   \includegraphics[width=\linewidth]{figures/compare.png}
   \caption{Results of 10$\times$ color upsampling on the 122\_smile model from the FaceScape dataset. \textbf{Best viewed zoomed in.}}
   \label{fig:compare}
\end{figure*}

\begin{figure*}[ht]
  \centering
   \includegraphics[width=\linewidth]{figures/mpeg.png}
   \caption{Results of 8$\times$ color upsampling on the LongDress model from the MPEG 8i dataset. }
   \label{fig:mpeg}
\end{figure*}
